PartNet: A Large-scale Benchmark for Fine-grained and Hierarchical Part-level 3D Object Understanding

We present PartNet: a consistent, large-scale dataset of 3D objects annotated with fine-grained, instance-level, and hierarchical 3D part information. Our dataset consists of 573,585 part instances over 26,671 3D models covering 24 object categories. This dataset enables and serves as a catalyst for many tasks such as shape analysis, dynamic 3D scene modeling and simulation, affordance analysis, and others. Using our dataset, we establish three benchmarking tasks for evaluating 3D part recognition: fine-grained semantic segmentation, hierarchical semantic segmentation, and instance segmentation. We benchmark four state-of-the-art 3D deep learning algorithms for fine-grained semantic segmentation and three baseline methods for hierarchical semantic segmentation. We also propose a novel method for part instance segmentation and demonstrate its superior performance over existing methods.

==> tex/intro_backup.tex <==
% benchmarking tasks: segmentation - recognition
% variety of methods for segmenting point clouds (citations)
% it's unclear how they would perform, and most them do not do instane level
% have a bit more citations for vision work to be more scholarly

% parts are critical for understanding world
Parts are critical for understanding the structure and semantics of objects in the real world.
People recognize, categorize, and organize objects according to their parts~\cite{hoffman1984parts}.
%Because parts compose to create functional objects, they are a key component of human knowledge underpinning our understanding of 3D shapes.
%Thus, part knowledge is important in many visual recognition tasks.
% 2D domain - datasets with part annotations
% vision cares about parts
In computer vision, the importance of parts has long been recognized ~\cite{nevatia1977description,marr1978representation},
%The seminal work of Marr and Nishihara~\cite{marr1978representation} represents objects as combinations of parametric part primitives.
with prior work leveraging part information for a variety of vision tasks such as recognition, detection, and classification ~\cite{felzenszwalb2008discriminatively,sun2011articulated,shrivastava2013building}.
Most recently, part segmentation tasks focus on segmenting objects into parts \cite{chen2014detect}.
However, much of this work is limited to the detection and reasoning of parts in 2D.

% In recent year, we are seeing the advent of 3D datasets and methods for 3D vision.
% People have realized that we need to move beyond 2D and start to have work in 3D vision
% to have useful part information need 3D parts and fine-grained parts
% Need to have more concrete examples (current work leveraging 3d shape parts)
% 3d - need 3d shape for manipulation and grasping
% For instance, knowing that a swivel chair has a base with 5 wheels, can aid in shape completion when occlusion is present.
Real objects and their parts exist in 3D.
Moreover, most actions that people (and robots) can take in the real world involve parts at a fine scale.
We open doors using door knobs, and we pick up mugs by grasping their handles.
These actions necessitate an understanding of the hierarchical connectivity and articulation of parts in real objects (door knobs turn and allow pulling open the door, mug handles move the whole mug and allow tilting to pour out liquids).
%Detecting fine-grained instance-level parts (e.g., door knobs, levers, and buttons) in 3D enables robotic grasping and manipulation.
Thus, many practical applications in robotics and manufacturing need to detect and reason about object parts \emph{hierarchically} at a \emph{fine-grained}, \emph{instance-level} in 3D.
%Representing fine-grained parts is important for the same reason (e.g. a robot needs to detect fine-grained parts such as door knobs, levers, buttons, etc.), and to allow generalization of knowledge between manufactured parts that together compose many real-world objects.
Understanding the hierarchical composition of parts from fine-grained components allows us to reason about the connectivity, articulation, and mobility of real objects (e.g., how the casters and wheels of an office chair allow it to spin and roll).


However, despite recent progress in constructing large scale 3D shape datasets such as ShapeNet~\cite{chang2015shapenet}, no existing dataset provides \emph{large-scale}, \emph{fine-grained}, \emph{hierarchical} part annotations.  
Prior work in 3D has only provided coarse part annotations on relatively small numbers of object instances~\cite{chen2009benchmark} or coarse, non-hierarchical part annotations~\cite{yi2016scalable}.
%Other work leverages existing incomplete part information to induce hierarchically parts at scale~\cite{yi2017learning}, however there is no consistently annotated ground truth part data at scale.
 To address this gap, we introduce \PARTS{}:
 a \emph{consistent, large-scale} dataset on top of ShapeNet with \emph{fine-grained, instance-level, hierarchical} 3D part information.

% 3D domain - datasets with parts either small or only have coarse grained parts
% datasets, lacking 3D fine-grained, hierarchical part annotations at scale
To ensure that parts are consistently labeled, we provide expert-defined \emph{template-hierarchies}.   With these templates we define parts consistently and at scale to enable the use of data-hungry deep learning methods.
These methods coupled with large-scale part data enable many applications including shape completion and shape synthesis. Here, we focus on three fundamental tasks for recognition: semantic segmentation, hierarchical segmentation, and instance-level segmentation.  We evaluate and benchmark recent methods for semantic segmentation on \PARTS{} and introduce novel methods for tackling hierarchical and instance-level segmentation.

%We provide several benchmark tasks to validate the dataset.

%To enforce consistency we use exper-defined part templates.

\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{fig/teaser.pdf}
   \caption{\textbf{PartNet dataset and its applications.} PartNet provides fine-grained and hierarchical instance-level part segmentation for 26,671 shapes from 24 object categories. Left: we show three example annotation in three levels of segmentation granularity defined in the hierarchy. Right: we propose three novel and challenging segmentation tasks and establish benchmarks using PartNet.}
   \label{fig:teaser}
\end{figure}

\begin{table*}[t]
  \centering
  \small
  \begin{tabular}[width=\linewidth]{c|cccccc}\Xhline{2\arrayrulewidth}
  \textbf{Dataset} &  \textbf{\#Shape}  &   \textbf{\#Category}  & \textbf{Granularity}     &  \textbf{Hierarchical}     & \textbf{Instance-level} &  \textbf{Consistent} \\ \Xhline{2\arrayrulewidth}
  \textbf{Chen et al.} \cite{chen2009benchmark} &  380   &  19    &   Fine-grained  & No  & Yes & No \\
  \textbf{MCL} \cite{wang2018learning} &   1,016 & 10   &  Fine-grained &  No  &  No   &  Yes  \\
  \textbf{Chang et al.} \cite{chang2018linking} & 1,021  &  90  &  Fine-grained  & No & Yes &  No \\
  \textbf{Yi et al.} \cite{yi2016scalable} &     31,963      &   16     &  Coarse  &  No  &  No  &  Yes  \\
  \hline
  \textbf{PartNet (ours)}    &   26,671      &  24   &     Fine-grained   &  Yes     &   Yes      & Yes         \\
    \Xhline{2\arrayrulewidth}
  \end{tabular}
  \caption{\textbf{Comparison to the Other Part Datasets.} }
  \label{tab:datacompare}
\end{table*}

In summary, we make the following contributions:
\begin{itemize}
\item We introduce the PartNet dataset, consisting of 573,585 fine-grained part annotations for 26,671 shapes across 24 object categories. To the best of our knowledge, it is the largest dataset with fine-grained and hierarchical instance-level part annotations.
\item We propose three part-level object understanding tasks to demonstrate the usefulness of this data: fine-grained semantic segmentation, hierarchical semantic segmentation, and instance segmentation.
\item We conduct extensive experiments to benchmark the tasks of fine-grained semantic segmentation and hierarchical semantic segmentation using PartNet.
\item We propose a novel method to address part instance-level segmentation and demonstrate state-of-the-art performance over the baseline method.
\end{itemize}





